Always Valid Inference: Bringing Sequential Analysis to A/B Testing

A/B tests are typically analyzed via frequentist p-values and confidence intervals; but these inferences are wholly unreliable if users endogenously choose samples sizes by *continuously monitoring* their tests. We define *always valid* p-values and confidence intervals that let users try to take advantage of data as fast as it becomes available, providing valid statistical inference whenever they make their decision. Always valid inference can be interpreted as a natural interface for a sequential hypothesis test, which empowers users to implement a modified test tailored to them. In particular, we show in an appropriate sense that the measures we develop tradeoff sample size and power efficiently, despite a lack of prior knowledge of the user's relative preference between these two goals. We also use always valid p-values to obtain multiple hypothesis testing control in the sequential context. Our methodology has been implemented in a large scale commercial A/B testing platform to analyze hundreds of thousands of experiments to date.

==> journal_multiple_old.tex <==
\section{Multiple Testing (old)}
\label{sec:multiple}

In A/B testing practice, it is often necessary to run multiple related experiments in parallel.  For instance, many treatments may be compared against a single control, or the treatments may be compared across multiple response metrics.  In this final section, we examine when always valid inference measures may be combined with common procedures from the {\em Multiple hypothesis testing} literature to ensure safe meta-experimentation in a sequential setting.  The methods presented have been deployed in the same A/B testing platform described in the preceding section.

For simplicity, we suppose that simple null hypotheses on some collection of parameters $\theta^1,...,\theta^m$ are tested, at each step one new observation is made in each experiment, and all the experiments are terminated simultaneously at an arbitrary stopping time that is adapted to the product of the $m$ corresponding filtrations so that some high-level decision can be made.  A naive approach is to construct always valid p-values and confidence intervals for each test individually.  This bounds the {\it False Positive Rate}: for any set of true parameters, for any stopping time, the expected proportion of the $m$ inference measures that incur false positives is at most $\alpha$. However, this guarantee may be insufficient for the experimenter to aggregate her results safely.

\subsection{p-values}

The goal of existing multiple testing procedures is to some achieve stricter Type I error control, which facilitates better decision-making.  For p-values, this means tighter control on the number of false positives among the {\it discoveries}: the set of null hypotheses that are rejected when the user thresholds each p-value at her chosen $\alpha$.  Most procedures in the literature take a set of fixed-horizon p-values as input and output a set of discoveries bounding one of two quantities at $\alpha$.  The first is on the {\em family-wise error rate} (FWER):
\begin{equation*}
\FWER  = \max_{\v{\theta}} \P_{\v{\theta}} (\delta_i = 1 \text{ for at least one } i \text{ s.t. } \theta^i = \theta_0^i ),
\end{equation*}
the worst-case probability of incurring any false positive.  It necessary to limit the FWER when one false discovery can derail decision-making; e.g. when comparing the treatment and control across multiple metrics, falsely concluding that the treatment performs well on just a single metric may motivate the experimenter to deploy the ineffective treatment.  The second quantity is the {\em false discovery rate} (FDR):
\begin{equation*}
\FDR = \max_{\v{\theta}} \E_{\v{\theta}} \left \{ \frac{ \# \{ 1 \leq i \leq m : \theta^i = \theta_0^i, \delta_i = 1 \} }{ \# \{ 1 \leq i \leq m : \delta_i = 1 \} \wedge 1 } \right \},
\end{equation*}
the worst-case expected proportion of discoveries that are false.  Bounding the FDR is appropriate for a user who weights all her significant results equally when making a decision, requiring only a set of discoveries that is ``mostly accurate".

In the sequential context, one would hope to apply the same procedures to a set of always valid p-values, and to achieve the desired bound at any data-dependent stopping time (on sample paths where this stopping time is infinite we consider the error incurred to be zero).  If a procedure satisfies this property for some class of always valid p-values, we say it {\em commutes with always validity} on that class.



%In this section, we combine always valid p-values and confidence intervals with standard procedures for {\em multiple hypothesis testing} to obtain more useful inferences for global decision-making.  In some contexts, new data may be collected for each experiment so that the p-value processes are independent, whereas sometimes it is desired to run many tests on overlapping data sets, inducing dependence in the corresponding p-value processes.  We address both cases here.

\subsection{Bonferroni and Benjamini-Hochberg}

%These procedures satisfy a transparency property that extends the transparency of fixed-horizon p-values described in the Introduction.  With multiple hypotheses, users may disagree on the global Type I error to be controlled, not just the level; nevertheless, different users can apply their chosen multiple testing correction to the same set of fixed-horizon p-values to achieve their desired global Type I error control.
%  For example, an overall planner may wish to bound FDR, while the tests may have been performed by many individual experimenters, each of whom aim to control only their per-experiment Type I error).  

%As ever, the purpose is to preserve transparency: no matter how the primary user chooses this stopping time, this enables a new user to apply their chosen multiple testing procedure to the p-values to obtain their desired Type I error control.  If a multiple testing procedure satisfies this property for a class of always valid p-values, we say it {\em commutes with always validity} on that class.

The standard procedure to control the FWER in the fixed-horizon context is the Bonferroni correction \cite{dunn1961multiple}: this rejects hypotheses $(1),...(j)$ where $j$ is maximal such that $p^{(j)} \leq \alpha/m$, 
and $p^{(1)},...,p^{(m)}$ are the p-values arranged in increasing order.  For FDR, the standard procedure is Benjamini-Hochberg \cite{benjamini1995controlling}. Two versions of BH are used, depending on whether the data are known to be independent across experiments.  If independence holds (BH-I), reject hypotheses $(1),...,(j)$ where $j$ is maximal such that $p^{(j)} \leq \alpha j / m$; in general (BH-G), choose the maximal $j$ such that:
\begin{equation*}
p^{(j)} \leq \frac{\alpha j}{m \sum_{r = 1}^m 1/r}.
\end{equation*}

Propositions \ref{prop:Bonferroni} and \ref{prop:bh_general} in Appendix \ref{sec:supp_multiple} establish that Bonferroni and the general form of BH commute with always validity on all p-value processes.  The reason is that, for any always valid p-values and any stopping time, the set of p-values evaluated at that time defines a set of fixed-horizon p-values.  BH-I does not commute with always validity over independent p-value processes, however, because stopping times that depend on every experiment can introduce correlation in the p-values at that time (see the Appendix for an example).  Nonetheless, for many natural choices of this stopping time, FDR control is still achieved for any independent always valid p-values.  Theorem \ref{thm:sequential_fdr} gives a sufficient condition on the stopping time.

%
%FDR control with BI-I does hold if some assumptions are placed on the stopping time.  To analyse this, we begin by defining some stopping times associated with the p-values that play a key role in our analysis.

\begin{definition}
Given independent always valid p-values $\v{p}_n$, let $S^{BH}_n$ be the rejections when BH-I is applied to these at level $\alpha$ and let $R^{BH}_n = |S^{BH}_n|$. Define:
\begin{equation} \nonumber
\begin{split}
&T_r = \inf \{ t \ : \ R_t^{BH} = r \}; \\
&T_r^{+} = \inf \{ t \ : \ R_t^{BH} > r \}; \\
&T_r^i = \inf \{ t \ : \ p_t^i \leq \frac{\alpha r }{m} \}. \\
\end{split}
\end{equation}

Now, if $p_{(1),n}^{-i}, p_{(2),n}^{-i},...$ are the p-values for the experiments other than $i$ placed in ascending order, consider a modified BH procedure that rejects hypotheses $(1),...,(k)$ where $k$ is maximal such that $p_{(k),n}^{-i} \leq \alpha (k+1)/m$, in parallel to the fixed horizon approach in \cite{benjamini1995controlling}.
Define the rejection set $(S^{BH}_n)^{-i}_0$ as those obtained under the original BH-I procedure if $p_n^i = 0$.  Let $(R^{BH}_n)^{-i}_0 = |(S^{BH}_n)^{-i}_0|$ and define:
\begin{equation} \nonumber
\begin{split}
&(T_r)^{-i}_0 = \inf \{ t \ : \ (R^{BH}_n)^{-i}_0 = r \} \\
&(T_r^+)^{-i}_0 = \inf \{ t \ : \ (R^{BH}_n)^{-i}_0 > r \} .
\end{split}
\end{equation}
\end{definition}

\begin{theorem}
\label{thm:sequential_fdr}
Given a stopping time $T$, let $m_0$ be the number of truly null hypotheses and let $I$ be the set of null hypotheses $i$ such that:
\begin{equation}
\label{eq:seq_fdr_requirement}
\sum_{r=1}^m \P \left( (T_{r-1})^{-i}_0 \ \leq \ T < (T_{r-1}^+)^{-i}_0 \ \Big| \  T_r^i \leq T \ , \ T < \infty \right) > 1
\end{equation}
Then the rejection set $S^{BH}_T$ has FDR at most
$$\alpha \left(\frac{m_0}{m} +  \frac{|I| \sum_{k=2}^m \frac{1}{k}}{m} \right).$$
In particular, if we permit only stopping times where $I$ is empty, BH-I controls FDR and so commutes with always validity over all independent processes.
\end{theorem}

\begin{proof}
We assume wlog that the truly null hypotheses are $i = 1,...,m_0$.  Letting $V_n$ denote the number of true null rejected at $n$, the FDR can be expanded as
\begin{equation} \nonumber
%\begin{split}
%&\E \left( \sum_{r=1}^m \ \frac{1}{r} \ V_T \ 1_{ \{ T_r \ \leq \ T < T_r^{+} \} }  1_{T < \infty}  \right) \\
%&= \E \left( \sum_{i=1}^{m_0} \sum_{r=1}^m \ \frac{1}{r} \ 1_{\{ T_r^i \leq T \}} \ 1_{ \{ T_r \ \leq \ T < T_r^{+} \} }  1_{T < \infty}  \right) \\
%&= \sum_{i=1}^{m_0} \sum_{r=1}^m \frac{1}{r} \P \left( T_r^i \leq T \ , \ T_r \ \leq \ T < T_r^{+} \ , \ T < \infty \right)
%\end{split}
\E \left( \sum_{r=1}^m \ \frac{1}{r} \ V_T \ 1_{ \{ T_r \ \leq \ T < T_r^{+} \} }  1_{T < \infty}  \right) = \sum_{i=1}^{m_0} \sum_{r=1}^m \frac{1}{r} \P \left( T_r^i \leq T \ , \ T_r \ \leq \ T < T_r^{+} \ , \ T < \infty \right).
\end{equation}
Note that the sets $ \{ T_r \ \leq \ T < T_r^{+} \} $ are disjoint and cover any location of $T$. Consider the terms in the sum over $i \in I$ and $i \notin I$ separately. For $i \notin I$, we bound the probability in the third equality by
\begin{equation} \nonumber
\begin{split}
\P \left( T_r^i \leq T \ , \ T < \infty \right)& \P \left(  T_r  \leq T < T_r^{+} \ \Big| \  T_r^i \leq T \ , \ T < \infty \right) 
 \leq \frac{\alpha r}{M}  \  \P \left(  T_r \leq T < T_r^{+} \ \Big| \  T_r^i \leq T \ , \ T < \infty \right) \\
 &= \frac{\alpha r}{M}  \  \P \left( (T_{r-1})^{-i}_0 \ \leq \ T < (T_{r-1})^{-i+}_0 \ \Big| \  T_r^i \leq T \ , \ T < \infty \right)
\end{split}
\end{equation}
where the first inequality follows from always-validity of sequential p-values, and the last equality because the modified BH procedure on the $m-1$ hypothesis other than the $i$th makes equivalent rejections at time $T$ when $T_r^i \leq T$. 

For $i \in I$, arguing as in the proof of Proposition \ref{prop:bh_general} shows
\begin{equation} \nonumber
%\begin{split} &\sum_{r=1}^m \frac{1}{r} \P \left( T_r^i \leq T \ , \ T_r \ \leq \ T < T_r^{+} \ , \ T < \infty \right) \\
%& \leq \frac{\alpha}{m} \sum_{k=1}^m \frac{1}{k}. 
%\end{split}
\sum_{r=1}^m \frac{1}{r} \P \left( T_r^i \leq T \ , \ T_r \ \leq \ T < T_r^{+} \ , \ T < \infty \right) \leq \frac{\alpha}{m} \sum_{k=1}^m \frac{1}{k}. 
\end{equation}
The proof is completed on application of (\ref{eq:seq_fdr_requirement}) to the terms in the first expansion with $i \notin I$ and re-ordering of the resulting terms.
\end{proof}

Perhaps the most natural stopping time for a user is the first time some fixed number $x \leq m$ hypotheses are rejected; i.e. $\ T = \inf_n \{ n \ : \ R_n = x \}$.  In that case,
\begin{gather*} 
\P \left( (T_{r-1})^{-i}_0 \ \leq \ T_x < (T_{r-1}^+)^{-i}_0 \ \Big| \  T_r^i \leq T_x \ , \ T_x < \infty \right)
= \P \left( (T_{r-1})^{-i}_0 \ \leq \ T_x < (T_{r-1}^+)^{-i}_0 \ \Big| \ T_x < \infty \right)
\end{gather*}
for each $i$.  This probability is 1 if $r = x$ and 0 otherwise, so $I$ is indeed empty and FDR is controlled.  On the other hand, a natural stopping time where $I$ is non-empty for some p-values is the first time that significance is reached in any of a given subset of experiments, where this subset has between two and $(m-1)$ elements.  A proof is given in the Appendix, together with simulations showing that FDR control can be violated in this case.


%Another very natural stopping time is the first time that the p-value on a fixed hypothesis crosses a threshold.  For both stopping times, we show next that $I$ is indeed empty. Example \ref{ex:rejecting_set} gives a case where $I$ may not be empty: stopping times where the user waits for rejection on a specific subset of hypotheses.
%
%\begin{example}[Rejection counts]
%\label{ex:first_rejection_counts}
%Suppose we want some number $x \leq m$ significant results to make a decision, and so stop at $\ T_x = \inf_n \{ n \ : \ R_n = x \}.$
%\begin{gather*} 
%\P \left( (T_{r-1})^{-i}_0 \ \leq \ T_x < (T_{r-1}^+)^{-i}_0 \ \Big| \  T_r^i \leq T_x \ , \ T_x < \infty \right)
%= \P \left( (T_{r-1})^{-i}_0 \ \leq \ T_x < (T_{r-1}^+)^{-i}_0 \ \Big| \ T_x < \infty \right)
%\end{gather*}
%for each $i$. This probability is 1 if $r = x$ and 0 otherwise.  Thus $I = \varnothing$, and so $FDR_{T_x}$ is at most $\alpha m_0 / m$.
%\end{example} 
%
%\begin{example}[Rejecting a single hypothesis]
%\[ T(j) = \inf \left \{ n \ : \ R_n > 0 \ , \ p_{j,n} \leq \frac{\alpha R_n}{m} \right \}. \]
%is the first time hypothesis $j$ is rejected.  By independence, for any $j$, again
%\begin{equation}\nonumber \begin{split} &\P \left( (T_{r-1})^{-i}_0 \ \leq \ T(j) < (T_{r-1}^+)^{-i}_0 \ \Big| \  T_r^i \leq T(j) \ , \ T(j) < \infty \right) \\
%= &\P \left( (T_{r-1})^{-i}_0 \ \leq \ T(j) < (T_{r-1}^+)^{-i}_0 \ \Big| \ T(j) < \infty \right).
%\end{split}
%\end{equation}
%Summing over $r$ we find that $I = \varnothing$.  Actually, FDR control in this example can be shown trivially without requiring Theorem \ref{thm:sequential_fdr}, since there is really only one hypothesis under consideration.
%\end{example}

\subsection{Recovering a simple interface}

In general, given any p-value in a given class, different users may apply any multiple testing procedure that commutes with always validity on that class to achieve their desired control.  However, this requires users to be statistically savvy. Alternatively, if we restrict our attention to just one of Bonferroni, BH-G or BH-I, we can recover the simple interface that p-values offer for single experiments by mapping the vector of p-values to a vector of {\em q-values} \citep{storey2003positive}.  Then the user only needs to threshold each $q^i$ at her chosen $\alpha$; $\v{q}$ is defined such that, for any $\alpha$, this policy obtains the same discoveries as applying the procedure to the p-values.  The mappings to obtain q-values are given in the appendix.

\subsection{Confidence intervals}

For p-values, multiple testing procedures ensure safe inference when the user focuses her attention on just discoveries.  Analogously, for confidence intervals, the goal is to control the number of false positives when the user focuses on some subset of the experiments determined by some data-dependent {\it selection rule}.  In this case, however, the rule is an {\em unknown property of the user}.  Whereas users typically only view the p-values of significant experiments, they may wish to gauge the range of plausible parameter values even in those where the null hypothesis is not rejected.

Firstly we note that, Bonferroni commutes with always validity for confidence intervals also.  That is, for any set of always valid confidence intervals $I^i_t(\alpha)$, we construct new intervals $I_t^i(\alpha/m)$.  These bound the FWER, the probability that a confidence interval fails to cover the true value on any of the selected experiments, uniformly over any selection rule.

%An FDR bound is designed to control the proportion of results that are false, when the user looks only at those experiments that achieve significance.  

The analogy to FDR is the {\em False Coverage Rate (FCR)} \cite{benjamini2005false}: the expected proportion of the selected confidence intervals that incur false positives, set at zero if none are selected.  \cite{benjamini2005false} gives a procedure to obtain FCR control at a fixed horizon when the selection rule is known: the nominal level $\alpha$ is replaced by $R\alpha/m$ for some $R$ defined in terms of the rule.  We begin by extending their approach to address unknown rules in the fixed-horizon context.

We restrict to selection rules that are the union of the discoveries and some fixed set $J$ of experiments, with $j = |J| \ll m$, which are always of interest to the user.  Theorem \ref{thm:fixed_horizion_FCR} then gives a procedure which bounds the FCR in terms of $j$.  The proof is given in the appendix.  For the procedure described in \cite{benjamini2005false}, it is the aggressive selection rules that choose few experiments which can obtain the highest FCR, and roughly speaking $R$ is a measure of how few experiments the rule can select.  Our approach is to be conservative over the unknown selection rule, taking $R$ for each interval to be the fewest number of experiments that could be selected, given that this interval corresponds to a selected experiment.

\begin{theorem}
\label{thm:fixed_horizion_FCR}
Given fixed-horizon p-values $\v{p}$, let $S^{BH}$ be the rejection set under BH-I, $R^{BH} = |S^{BH}|$, and $(CI^i(1-s))_{i =1}^m$ be the corresponding fixed-horizon CIs at each level $s \in (0,1)$.  Define the corrected confidence intervals:
\begin{equation}
\tilde{CI}^i =
\begin{cases}
CI^i(1-R^{BH}\alpha / m) & i \in S^{BH};\\
CI^i(1-(R^{BH}+1)\alpha / m) & i \notin S^{BH}.
\end{cases}
\end{equation}
Then for any $J$, if the selection rule is the experiments $J \cup S_{BH}$, the FCR is at most $\alpha(1 + j/m)$.
\end{theorem}

In the sequential setting, CI processes that give approximate FCR control can be derived from always valid p-values analogously, provided we make restrictions on the stopping time similar to those required for FDR control. 
\begin{definition}
If $p_n^{i, \theta_0}$ is the p-value for testing $H_0: \theta^i = \theta_0$, let
\begin{align*}
&T_r^{i,\theta_0} = \inf \{ t \ : \ p_t^{i, \theta_0} \leq \frac{\alpha r }{m} \}\\
&(T_r)^{-i, J}_0 = \inf \{ t \ : \ |(S^{BH}_n)^{-i}_0 \cup J \backslash i| = r \} \\
&(T_r^+)^{-i, J}_0 = \inf \{ t \ : \ |(S^{BH}_n)^{-i}_0 \cup J \backslash i| > r \} .
\end{align*}
The last two stopping times denote the first times at least $r$ and more than $r$ experiments other than $i$ are selected.

If $p_{(1),n}^{-i}, p_{(2),n}^{-i},...$ are the p-values for the experiments other than $i$ placed in ascending order, consider another modified BH procedure that rejects hypotheses $(1),...,(k)$ where $k$ is maximal such that
$$ p_{(k),n}^{-i} \leq \alpha \frac{k}{m}, $$
These are the rejections obtained under the original BH-I procedure if $p_n^i = 1$.  We define stopping times associated with this procedure $(T_r)^{-i,J}_1$ and $(T_r^+)^{-i,J}_1$ analogous to the two stopping times above.
\end{definition}

\begin{theorem}
\label{thm:sequential_FCR}
Given independent always valid p-values $\v{p}_n$ and corresponding CIs $(CI_n^i(1-s))_{i =1}^m$ at each level $s \in (0,1)$.  Define new confidence intervals
\begin{equation}
\tilde{CI}_n^i =
\begin{cases}
CI_n^i(1-R_n^{BH}\alpha / m) & i \in S^{BH}_n\\
CI_n^i(1-(R_n^{BH}+1)\alpha / m) & i \notin S^{BH}_n
\end{cases}
\end{equation}
Let $J$ be a set of experiments and let $T$ be a stopping time such that the following conditions hold for every $i$, where $\theta^i$ is the true parameter value for that hypothesis:
\begin{align}
\sum_{r = 1}^m \P((T_r)^{-i, J}_0 \leq T < (T_r^+)^{-i, J}_0 | T_r^{i,\theta^i} \leq T < \infty) \leq 1\\
\sum_{r = 1}^m \P((T_r)^{-i, J}_1 \leq T < (T_r^+)^{-i, J}_1 | T_r^{i,\theta^i} \leq T < \infty) \leq 1
\end{align}
Then under the selection rule $J \cup S^{BH}_T$, the intervals $(\tilde{CI}_T^i)$ have FCR at most $\alpha(1 + j/m)$.
\end{theorem}

The Bonferroni-corrected CIs and the FCR-controlling CIs defined in the above theorem are each displayed in the industry platfrom in appropriate contexts.

%{\bf Simulations.} To test the slack in the $\FDR$ bounds, we ran mSPRT tests on the location parameter of normal data with known variance $\sigma^2 = 1$, normal mixture, and mixing parameter $\tau^2 = 1/100$ up to a maximum sample size of $n_{max}=50,000$. In each case, $M$ tests were run with $\pi_0$ proportion null ($\theta=0$), to which we applied the BH-I procedure at three stopping times, $T^{\cup}(\{1,\dots,k\})$, $T^{\cap}(\{1,\dots,k\})$, and $T_k$, where the first $\pi_0 M$ are null and the rest non-null.

%Figure \ref{fig:fdr_sim} shows results. We find that \eqref{eq:tcup_bound} is an upper bound for $\FDR$ in all cases and is most tight for $T_1 = T^{\cup}(\{1,\dots,m\})$, or the ``first rejection time.'' The largest inflation of $\FDR$ was about $.16$ for $M=100$, $\pi_0 = .79$ and a \emph{lo effect} size for $T^{\cup}(\{1,\dots,79\})$, while \eqref{eq:tcup_bound} was almost double at $.29$. 

%%%%%
%In each case, $M$ tests were run with $\pi_0$ proportion null ($\theta=0$). The remaining $1-\pi_0$ proportion were run with either a \emph{low effect}, defined as the effect size with expected sample size of roughly $n_{max}$, or \emph{hi effect}, defined as the effect size with expected sample size equal to the $n_{.1}$ where $\P_0 \left( p_{n_{.1}} \leq \alpha \Big| p_{n_{max}} \leq \alpha \right) = .1$. To calculate these values of $\theta$, we used the the approximations in \cite{LS1979} and \cite{LS77}. The $\pi_0$ cases considered were $.1$, $.5$, $.9$ and the value which maximizes \eqref{eq:tcup_bound} for a given $M$.

%Each multiple $mSPRT$ run gave a $M \times n_{max}$ matrix of p-values, to which we applied the BH procedure at three stopping times, $T^{\cup}(\{1,\dots,k\})$, $T^{\cap}(\{1,\dots,k\})$, and $T_k$, where the first $\pi_0 M$ are null and the rest non-null, and calculated the $Fdp$. Finally, $B=1000$ replications gave an estimate of $\FDR$. We set $\alpha = .1$ in all cases.

%\begin{figure}[h!] 
%  \centering
%    \includegraphics[width=\textwidth]{../img/sfdr_simulation_results_nic} 
%    \caption{Sequential $\FDR$ is estimated from running mSPRT tests on the location parameter of normal data with known variance $\sigma^2 = 1$, normal mixture, and mixing parameter $\tau^2 = 1/100$ up to a maximum sample size of $n_{max}=50,000$, and applying the BH-I procedure at three stopping times: $T^{\cup}(\{1,\dots,k\})$ ($\circ$), $T^{\cap}(\{1,\dots,k\})$ ($\bigtriangleup$), $T_k$ ($\times$). The x-axis indexes the hypothesis id $k$, where the first $p_0 \times M$ hypotheses are nulls, and the remaining non-nulls, as indicated by the vertical pink line. The y-axis is an estimate of $\FDR$ from $1000$ replications of running $M$ mSPRTs and applying BH-I at the prescribed stopping time. In each case, the $1-\pi_0$ proportion were run with either a \emph{low effect}, defined as the effect size with expected sample size of roughly $n_{max}$, or \emph{hi effect}, defined as the effect size with expected sample size equal to the $n_{.1}$ where $\P_0 \left( p_{n_{.1}} \leq \alpha \Big| p_{n_{max}} \leq \alpha \right) = .1$. The $\pi_0$ cases considered were $.1$, and $.9$. We find that the bound in \eqref{eq:tcup_bound} holds in all cases, and is most tight for $T_1 = T^{\cup}(\{1,\dots,m\})$, the ``first rejection time.''}
%\label{fig:fdr_sim}
%\end{figure}


==> journal_optimality.tex <==
\section{Optimal p-value processes}
\label{sec:optimality}

As noted in the preceding section, users who continuously monitor experiments are making a dynamic tradeoff between two objectives: detecting true effects with maximum probability and minimizing the typical length of experiments.  A significant challenge for the platform is that always valid p-values must be designed without prior knowledge of the user's preferences.  We are led, therefore, to consider the following design problem: how should always valid p-values be designed to lead users to a near-optimal tradeoff between power and run-length, without access to the user's preferences in advance?

In this section we first introduce a natural model of user behavior that encodes a tradeoff between power and run-length.  Then we consider always valid p-value processes derived from a particular family of sequential tests, the {\em mixture sequential probability ratio tests} (mSPRT), proving that any mSPRT provides near-optimal decision making for all of these users simultaneously.  Specifically, for any such user, it is not possible to improve detection uniformly at every effect size in the limit as $\alpha \to 0$.  Moreover, we optimize among mSPRTs for average-case performance when prior knowledge on the effect size sought is available, and we establish an improvement over fixed-horizon testing in that case.  The proofs are given in Appendix \ref{sec:supp_optimality}.

\subsection{The user model}

Of course, any specific user's preferences will be highly nuanced.  In our analysis, for technical simplicity we consider the following user model: we assume users can be characterized by a parameter $M$ representing the maximum number of observations that the user is willing to wait, together with their Type I error tolerance $\alpha$.  Given an always valid p-value process, we consider a simple model of user behavior: users stop at either the first time the p-value drops below $\alpha$ (in which case they reject the null), or at time $M$ (in which case they do not reject the null unless the p-value at time $M$ is also below $\alpha$), whichever occurs first.

We refer to such a user as a {\em $(M,\alpha)$ user}.  In the remainder of the section, our goal will be to make near-optimal tradeoffs between power and run-length for $(M,\alpha)$ users in the limit where $\alpha \to 0$, without prior knowledge of their preferences.  We note the following technical remark: if the always valid p-values shown to a user are derived from a sequential test $(T(\alpha), \delta(\alpha))$, then the $(M,\alpha)$ user's decision rule is given by $T(M, \alpha) \triangleq \min\{ T(\alpha), M \}$, and $\delta(M, \alpha) = 1$ if and only if $T(\alpha) \leq M$.

\subsection{The mSPRT}

The always valid p-values we employ are derived from a particular family of sequential tests: the {\em mixture sequential probability ratio test} (mSPRT) \citep{robbins1970statistical}.  We begin by imposing slight restrictions on the data model: we assume that the data is real valued and drawn from a single parameter exponential family, $f_\theta(x) = F'_\theta(x) = f_0(x) \exp(\theta x - \psi(\theta))$, where tests are of the natural parameter $\theta$, $\Theta$ is an open interval, $\psi^{''}(\theta) > 0$ for all $\theta$, and $\E|X_1|^p < \infty$ for some $p \geq 4$.

The mSPRT is parameterized by a {\em mixing distribution} $H$ over $\Theta$, which we restrict to have everywhere continuous and positive derivative. Given an observed sample average $s_n$ up to time $n$, the likelihood ratio of $\theta$ against $\theta_0$ is $(f_\theta(s_n)/f_{\theta_0}(s_n))^n$.  Thus we define the {\em mixture likelihood ratio} with respect to $H$ as
\begin{equation} \label{eq:msprt_definition} \Lambda_n^H(s_n) = \int_{\Theta} \left( \frac{f_\theta(s_n)}{f_{\theta_0}(s_n)}\right)^n dH(\theta).
\end{equation}
The mSPRT is then defined by:
\begin{align}
T^H(\alpha) & = \inf\{n : \Lambda_n^H(S_n) \geq \alpha^{-1} \}; \ \ \text{and} \label{eq:mSPRT1}\\
\delta^H(\alpha) &= \1 \left\{T^H(\alpha) < \infty\right\}, \label{eq:mSPRT2}
\end{align}
where $S_n = \sum_{i=1}^n X_i$.  The choice of threshold $\alpha^{-1}$ on the likelihood ratio ensures Type I error is controlled at level $\alpha$, via standard martingale techniques \citep{siegmund1985sequential}. Intuitively, $\Lambda_n^H(S_n)$ represents the evidence against $H_0$ in favor of a mixture of alternative hypotheses, based on the first $n$ observations. The test rejects $H_0$ if the accumulated evidence ever becomes large enough.	
%We model such a user's choice of stopping time by $T(M, \alpha) = T(\alpha) \wedge M$. So, if we provide the p-value associated with some test $(T(\alpha), \delta(\alpha))$, she implements the truncated sequential test $(T(M, \alpha),\delta(M, \alpha) = 1(T(\alpha) \leq T(M, \alpha))$ upon stopping. 
%
%Given a p-value process, we suppose that the user selects a stopping time $T$ that reflects her priorities for maximizing power while minimizing run-length. In so doing, she implements a new sequential test that is derived from the sequential test $(T(\alpha), \delta(\alpha))$ associated with that p-value. Thus, optimizing the choice of p-value means simultaneously optimizing the derived sequential test that each user obtains.

Our first motivation for considering mSPRTs is that they are {\em tests of power one} \citep{RS74}: for all $\alpha$ and $\theta \neq \theta_0$, there holds:, 
\[  \P_\theta( T(\alpha) < \infty, \delta(\alpha) = 1) = 1. \]
In other words, for the hypothetical user who can wait forever, any mSPRT delivers power one for any alternative.  We also note here that in a Bayesian setting where the user's cost function takes a suitable linear form and the stopping time and $\alpha$ are fixed optimally, mSPRTs are known to be optimal in terms of Bayes risk in a suitable limit \citep{lai2001sequential}.\footnote{This limit maps to the setting where $\alpha \to 0$, where we also focus attention in our results.}

%% any mSPRT uniformly optimizes both : for $M = \infty$, the relative run-length profile is everywhere zero (trivially), while power is everywhere one. Secondly, when This limit is analogous to the limit $\alpha \to 0$ we address

For later reference, we note the following result due to \cite{PS1975}: for any mixing distribution $H$, as $\alpha \to 0$,
\begin{equation}
\label{eq:limit_prob}
T^H(\alpha) / \log(1/\alpha) \to I(\theta, \theta_0)^{-1} := \left \{ (\theta - \theta_0) \psi'(\theta) - (\psi(\theta) - \psi(\theta_0)) \right \}^{-1}
\end{equation}
holds in probability and in $\mathcal{L}^2$, where $\psi(\theta)$ is the log-partition function for the family $F_\theta$.  This result characterizes the run-length of the mSPRT in the small $\alpha$ limit, and plays a key role in our subsequent study of efficiency.

\subsection{Efficiency in the $\alpha \to 0$ limit}

We now formalize our study of the power and run-length tradeoff for an $(M, \alpha)$ user.  To proceed, suppose that the way this user makes decisions is to use a rule $(T^*, \delta^*)$ that controls Type I error at level $\alpha$ (i.e., $\P_{\theta_0}(\delta^* = 1) \leq \alpha$), and satisfies the constraint that $T^* \leq M$ a.s.  We refer to such decision rules as {\em feasible} decision rules for an $(M, \alpha)$ user.  

We first map the two objectives of the user to formal quantities of interest.  First, an $(M, \alpha)$ user will want to choose her decision rule to maximize the {\em power profile} $\nu(\theta) = \P_\theta(\delta^* = 1)$ over $\theta \neq \theta_0$. Second, she will want to minimize the {\em relative run-length profile} of relative run-lengths measured against the maximum available to her, $\rho(\theta) = \E_\theta(T^*) / M$.

{\em Perfect efficiency} would entail $\rho(\theta) = 0$ and $\nu(\theta) = 1$ for all $\theta \neq \theta_0$.  Of course, perfect efficiency is generally unattainable.  In this section we study the best achievable performance such a user can hope for, in the limit where $\alpha \to 0$.

Our analysis depends on the characterization of run-length of the mSPRT in \eqref{eq:limit_prob}.  The consequence is that if we produce always valid p-values using the mSPRT, then in the $\alpha \to 0$ the study of efficiency divides into three cases depending on the relative values of $M$ and $\log(1/\alpha)$.  We consider these cases in turn.

{\bf ``Aggressive'' users: $M \gg \log(1 / \alpha)$.} Users in this regime are aggressive; $\alpha$ is large relative to the maximum run-length they have chosen.  In this regime, any mSPRT asymptotically recovers perfect efficiency in the limit where $\alpha$ small.  Intuitively, because the user is willing to wait a substantially longer time than $\log(1/\alpha)$, a sublinear fraction of their maximum run-length is used by the mSPRT; since the mSPRT is a test of power 1, this means the user receives power near 100\% in return for a near-zero run-length profile.  The proof of the following result follows immediately from (\ref{eq:limit_prob}).
\begin{proposition}
	Given any mixture $H$, let $\rho(\theta)$ and $\nu(\theta)$ be the relative run-length and power profiles, respectively, associated with $(T^H(M, \alpha), \delta^H(M, \alpha))$. If $\alpha \to 0$ and $M \to \infty$ such that $M/\log(1/\alpha) \to \infty$, we have $\rho(\theta) \to 0$ and $\nu(\theta) \to 1$ at each $\theta \neq \theta_0$.
\end{proposition}

{\bf ``Conservative'' users: $M \ll \log(1 / \alpha)$.}  Users in this regime are conservative; $\alpha$ is small relative to the maximum run-length they have chosen.  In this case, experimentation is not productive: the user is unwilling to wait long enough to detect any effects.  Thus any mSPRT trivially performs as well as any feasible decision rule for the user.
\begin{proposition}
\label{prop:conservative}
	For each $(M, \alpha)$, let $(T^*(M, \alpha), \delta^*(M, \alpha))$ be any test such that $T^* \leq M$ a.s. and $\nu^*(\theta_0) \leq \alpha$, where $\nu^*$ is the associated power profile. Then if $\alpha \to 0, M \to \infty$ such that $M/\log(\alpha^{-1}) \to 0$, we have $\nu^*(\theta) \to 0$ for each $\theta$.
\end{proposition}

{\bf ``Goldilocks'' users: $M \sim \log(1 /\alpha)$.}  This is the interesting case, where experimentation is worthwhile but statistical analysis is non-trivial.  To proceed we require an additional definition.  For a family of sequential tests, we define the worst-case efficiency over $\theta \neq \theta_0$ for a user with parameters $(M, \alpha)$ as the relative efficiency of the truncated test they obtain by minimizing the relative run-length everywhere, compared with any other test that offers at least as good power everywhere.  This is formalized as follows.

\begin{definition}
	Given a sequential test $(T(\alpha), \delta(\alpha))$, let $\rho(\theta; \alpha, M)$ and $\nu(\theta; \alpha, M)$ be the relative run-length and power profiles associated with $(T(M, \alpha), \delta(M, \alpha))$. The {\em relative efficiency} of this test at $(M, \alpha)$ is
\[ \phi(M, \alpha) = \inf_{(T^*, \delta^*)} \inf_{\theta \neq \theta_0} \frac{\rho^*(\theta)}{\rho(\theta; \alpha,M)} \]
where the infimum is taken over feasible tests (i.e., $T^* \leq M$ a.s.~and $\P_{\theta_0}(\delta^* = 1) \leq \alpha$) such that for all $\theta \neq \theta_0$ there holds $\nu^*(\theta) \geq \nu(\theta; \alpha, M)$.
\end{definition}

Our main result demonstrates that in the regime where $M \sim \log(1/\alpha)$, any mSPRT has relative efficiency approaching unity when $\alpha \to 0$.

\begin{theorem}
\label{thm:efficiency}
	Suppose $\psi''$ is absolutely continuous and there is an open interval around $\theta_0$ where $\psi''(\theta) < \infty$. Given any $H$, let $\phi(M, \alpha)$ be the efficiency of the mSPRT $(T^H(\alpha), \delta^H(\alpha))$. If $\alpha \to 0, M \to \infty$ such that $M = O(\log(\alpha^{-1}))$, we have $\phi(M, \alpha) \to 1$.
\end{theorem}


%%  We show that for a family of tests - mixture Sequential Probability Ratio Tests (mSPRTs) - an efficient trade off is obtained between these profiles in a worst-case sense over $\theta$, in the limit $\alpha \to 0$. Crucially, this efficiency is obtained simultaneously for any user; i.e. for all $M$. To select among mSPRTs, some knowledge about typical effect sizes is required. We identify the optimal mSPRT to minimize the average relative run-length when a prior for $\theta$ under $H_1$ is available.

%% In this section, 

%% %[PUT IN BACKGROUND SECTION] We note here that, although tests that incorporate truncation at some specified $n_S$ have been studied extensively, e.g. \cite{siegmund1985sequential} Ch. 3 \& 4, the construction of tests that perform well at any user-selected $n_S$ is a novel objective necessitated by the demands of A/B testing.

%% {\bf mSPRTs.} 

%{\bf $M << I(\theta, \theta_0)^{-1} \log(1 / \alpha)$.}  {\bf $M = O(\log(1 / \alpha))$.} 
%{\bf Power at $n_S = \infty$.} To serve users who will wait an arbitarily long time, we demand that any true effect is ultimately detectable. That is, we restrict to so-called \emph{tests of power one} \cite{RS74}, where
%$$ \forall \alpha, \theta \neq \theta_0, \,\, \P_\theta( T(\alpha) < \infty, \delta(\alpha) = 1) = 1.$$
%
%{\bf Trade-off as $n_S \to \infty$.} Next we say that a test of power one $(T(\alpha), \delta(\alpha))$ is \emph{$\epsilon$-efficient at $(n_S, \alpha)$} if
%\begin{equation}
%\label{eq:efficiency_speed}
%\forall \theta \neq \theta_0, \,\, \E_\theta (T_{n_S}^\alpha) < \E_\theta (T^*) (1 + \epsilon)
%\end{equation}
%for any test $(T^*, \delta^*)$ with Type I error at most $\alpha$, and Type II error satisfying
%\begin{equation}
%\label{eq:efficiency_power}
%\forall \theta \neq \theta_0, \,\, \P_\theta (\delta^* = 0)(1 + \epsilon) \leq \P_\theta (\delta_{n_S}^\alpha = 0).
%\end{equation}
%$\epsilon$-efficiency means that, even with knowledge of $n_S, \alpha$, it is not possible to reduce the expected run time at some $\theta$ without comprimising on power at some $\theta'$. As $n_S \rightarrow \infty$, we suppose that $\alpha(n_S) \to 0$; if the user can wait long to achieve high power, they can reasonably demand vanishing Type I error. Theorem \ref{thm:optimal_trunc_msprt} shows that every mSPRT (see below) becomes arbitrarily efficient in the limit $n_S \to \infty$, provided $\alpha(n_S)$ cannot approach 0 too quickly. If it does, the user becomes too conservative to detect true effects with any test.
%
%The mSPRT \cite{robbins1970statistical} are a class of sequential tests, parameterized by an mixing distribution $H$ over $\Theta$, assumed to have continuous and positive derivative in a neighborhood of the true $\theta$. For the set of mixture likelihood ratios,
%\begin{equation} \label{eq:msprt_definition} \Lambda_t^H(x) = \int_{\Theta} \frac{f_\theta(x)}{f_{\theta_0}(x)} dH(\theta) 
%\end{equation}
%the test is defined by $T^H(\alpha) = \inf\{n : \Lambda_n^H(S_n) \geq \alpha^{-1} \}$ and $\delta^H_{\alpha} = 1(T^H(\alpha) < \infty)$, where $S_n = \sum_{i=1}^n X_i$. \footnote{The choice of threshold $\alpha^{-1}$ on the likelihood ratio ensures Type I error is controlled at level $\alpha$, via standard martingale techniques \cite{siegmund1985sequential}.} These are tests of power one \cite{RS74} as we require. We are motivated to consider these tests, because when the user's cost function takes a suitable linear form and the stopping time and $\alpha$ are fixed optimally, mSPRTs are known to be optimal in terms of Bayes risk in a similar data-cheap limit. \cite{lai2001sequential}
%
%We begin by stating a useful result of \cite{PS1975}: for any $H$, as $\alpha \to 0$,
%\begin{equation}
%\label{eq:limit_prob}
%T^H(\alpha) / \log(\alpha^{-1}) \to I(\theta, \theta_0)^{-1} := \left \{ (\theta - \theta_0) \psi'(\theta) - (\psi(\theta) - \psi(\theta_0)) \right \}^{-1}
%\end{equation}
%holds in probability and in $\mathcal{L}^2$, where $\psi(\theta)$ is the log-partition function for the family $F_\theta$.
%
%\begin{theorem} \label{thm:optimal_trunc_msprt}
%Suppose $\psi''$ is absolutely continuous, there is an open interval around $\theta_0$ where $\psi''(\theta) < \infty$, and $H'$ is continuous and positive over all $\Theta$.  Let $\epsilon > 0$, and $(n_S^k, \alpha^k)_{k=1}^\infty$ be an arbitrary sequence approaching $(\infty, 0)$. If $\log \{ (\alpha^k) ^{-1} \} / n_S^k$ is bounded, $(T^H(\alpha), \delta^H(\alpha))$ is $\epsilon$-efficient at $(n_S^k, \alpha^k)$ for all $k$ sufficiently large.
%
%On the other hand, suppose that $\log \{ (\alpha^k) ^{-1} \} / n_S^k \to \infty$ and $(T,\delta)$ is any test satisfying $\P_{\theta_0}(\delta_{n_S^k}^{\alpha^k} = 0) \leq \alpha^k$. Then $\delta_{n_S^k}^{\alpha^k} \stackrel{p}{\to} 0$ under any $\theta$, so no detection is possible.
%\end{theorem}

%\rj{Move proof to appendix}
%\begin{proof}
%Since the family $F_\theta$ can be equivalently viewed as exponential tilts of any $\theta' \in \Theta$, we assume $\theta_0 = 0$ wlog and write $I(\theta) := I(\theta,0)$. Using the normal approximation from Theorem 2 of \cite{LS77} gives
%\[\P_\theta ( \delta_{n_S^k}^{\alpha^k} = 0 ) = \bar{\Phi} \left\{ \log \{ (\alpha^k)^{-1} \}^{1/2} B_k(\theta) \right\}(1 + o(1) )\]
%as $k \to \infty$, where $B_k(\theta) = \left( \frac{ I(\theta)^3 }{\theta^2 \psi^{''}(\theta)} \right)^{1/2} \left( \frac{ n_S^k }{ \log \{ (\alpha^k)^{-1} \} } - I(\theta)^{-1} \right).$
%Standard results on the log partition function $\psi$ imply that for any $k$, under the given assumptions,
%$$ \log \{ (\alpha^k)^{-1} \}^{1/2} B_k(\theta) \sim \eta_2 \log \{ (\alpha^k)^{-1} \}^{1/2} \left(  \frac{ n_S^k }{ \log \{ (\alpha^k)^{-1} \} } \, \theta^2 - \eta_2 \right) $$
%as $\theta \rightarrow 0$, where $\eta_2$ and $\eta_3$ are both positive constants. Hence, if $\log \{ (\alpha^k) ^{-1} \} / n_S^k$ is bounded, for $k$ large enough we can choose $\theta_1^k = \sqrt{\frac{\log \{ (\alpha^k)^{-1} \}}{n_S^k} ( \sqrt{2 / \eta_2} + \eta_3 )} \in \Theta$ such that
%$$ \bar{\Phi} \left\{ \log \{ (\alpha^k)^{-1} \}^{1/2} B_k(\theta) \right\}(1 + o(1) ) = \bar{\Phi}\left( \sqrt{2 \log \{ (\alpha^k)^{-1} \} } \right) := \beta_1^k $$
%Let $(T^*_k, \delta^*_k)$ be a test with Type I error at most $\alpha^k$ and Type II error at $\theta_1^k$ at most $\beta_1^k$, and consider $k$ large enough such that $0 < \alpha^k + \beta_1^k < 1$. Then by Hoeffding's inequality, for any $\theta \notin \{ 0, \theta_1^k \}$, we have
%\begin{align*}
%\E_\theta(T^*_k) &\geq \frac{ | \log( \alpha^k + \beta_1^k) | - \frac{1}{2} \theta_1^2 \psi''(\theta)  | \log( \alpha^k + \beta_1^k) |^{1/2} }{\max\{ I(\theta), I(\theta,\theta_1) \}}\\
%&= I(\theta)^{-1} \log \{ (\alpha^k)^{-1} \} (1 + o(1) )
%\end{align*}
%By continuity, the result holds at $\theta_1^k$ also. Thus, given $\epsilon > 0$, (\ref{eq:efficiency_speed}) holds for $k$ sufficiently large by comparing the above expression with (\ref{eq:limit_prob}).
%
%Now we address the case $\log \{ (\alpha^k) ^{-1} \} / n_S^k \to \infty$. Let $\beta < 1$ be arbitrary and consider $k$ large enough that $\alpha^k + \beta < 1$. Given any $\theta$, suppose that $\P_{\theta}(\delta_{n_S^k}^{\alpha^k} = 0) \geq \beta$. Combining this with $\P_0(\delta_{n_S^k}^{\alpha^k} = 0) \leq \alpha^k$, the Hoeffding inequality implies the existence of some $\kappa$ such that
%\[ \E_\theta(T^{\alpha^k}_{n_S^k}) \geq \kappa \log \{ (\alpha^k)^{-1} \} (1 + o(1)) \]
%For $k$ sufficiently large, this expression is strictly greater than $n_S^k$, which gives a contradiction.
%\end{proof}

\subsection{Run-length optimization}

Now we go one step further and optimize our choice of mSPRT.  As noted in the preceding section, it is users with $M \sim \log(1/\alpha)$ where there is a meaningful tradeoff between run-length and power, and for these users any mSPRT is asymptotically efficient as $\alpha \to 0$.  That is, no mSPRT can offer a uniform improvement at every $\theta$ in that limit.  However, the choice of $H$ governs a tradeoff between performance at different effect sizes.  We now consider a Bayesian setting where we have a prior $\theta \sim G$ under $H_1$.  The following theorem gives the mixing distribution $H$ that minimizes the relative run-length on average over this prior for a ``goldilocks" user with parameters $(M, \alpha)$.

\begin{theorem} \label{thm:optimal_mixture}
Suppose $G$ is absolutely continuous with respect to Lebesgue measure, and let $H_\gamma$ be a parametric family, $\gamma \in \Gamma$, with density $h_\gamma$ positive and continuous on $\Theta$. Let $\rho_\gamma(\theta)$ be the profile of relative run-lengths associated with $(T^{H_\gamma}(M, \alpha), \delta^{H_\gamma}(M, \alpha))$. Then up to $o(1)$ terms as $\alpha \rightarrow 0, M = O(\log(1/\alpha))$, the average relative run-length $\rho_\gamma(M,\alpha) = \E_{\theta \sim G} \{\rho_\gamma(\theta)\}$ is minimized by any $\gamma^*$ such that:
\begin{equation} \label{eq:prior_matching} \gamma^* \in \argmin_{\gamma \in \Gamma} - \E_{\theta \sim G} \v{1}_{A(M, \alpha)} I(\theta, \theta_0)^{-1} \log h_\gamma(\theta), \end{equation}

where $A(M, \alpha) = \left \{ \theta : I(\theta, \theta_0) \geq\log (1/\alpha) / M \right \}$.

If $h_\gamma(\theta) = q(\gamma_1,\gamma_2) e^{\gamma_1 \theta - \gamma_2 \psi(\theta)}$, a conjugate prior for $f_\theta$, then $\gamma^*$ solves:

\[ \frac{ \partial q(\gamma_1,\gamma_2) / \partial \gamma_1}{\partial q(\gamma_1, \gamma_2) / \partial \gamma_2} = \frac{ \E_{\theta \sim G} \v{1}_A \theta I(\theta, \theta_0)^{-1}}{\E_{\theta \sim G} \v{1}_A \psi(\theta) I(\theta, \theta_0)^{-1}}. \]

Optimizing for $h_\gamma$ does not impact first order terms of $\E_{\theta \sim G} \{\rho_\gamma(\theta)\}$ in this limiting regime.
\end{theorem}

Heuristically, the mSPRT rejects $H_0$ when there is sufficient evidence in favor of any $H_1 : \theta \neq \theta_0$, weighted by the distribution $H$ over alternatives. Thus we might expect optimal sampling efficiency when $H$ is {\em matched} to the prior. If we specialize to normal data, $f_\theta(x) = \phi(x-\theta)$, a centered normal prior, $G(\theta) = \Phi(\frac{\theta}{\tau})$, and consider normal mixtures, $h_\gamma(\theta) = \frac{1}{\gamma} \phi(\frac{\theta}{\gamma})$, this intuition is mostly accurate.  In that case, the optimal choice of mixing variance becomes:
\begin{equation}  \label{eq:prior_matching_normal} \gamma^{2*} = \tau^2 \frac{ \Phi(-b) }{ \frac{1}{b} \phi(b) - \Phi(-b)}
\end{equation}
for $b = \left( \frac{2 \log \alpha^{-1} }{M \tau^2} \right)^{1/2}$. In fact, this is equal to the prior variance multiplied by a factor correcting for anticipated truncation that depends on $M$. Sampling efficiency is improved by weighting towards larger effects when few samples are available and smaller effects where there is ample data.

Nominally, this truncation correction presents a challenge: it appears the optimal mixture distribution depends crucially on $M$.  However, as we now demonstrate both empirically and through simulation, the choice of mixing distribution is quite robust with respect to variation in $M$.  From our numerical analysis of over $40,000$ historical A/B tests on a leading industry platform (see Section \ref{sec:abtests}) we were able to construct a prior for $\theta$ under $H_1$ for experiments run on that platform. We found that, given $\alpha$ and $M$,  the choice of $H$ given by (\ref{eq:prior_matching_normal}) provides a substantial reduction in the average run time over highly suboptimal choices of $\gamma^2$ (optimizing $H$ is worthwhile).  However, a single choice of $\gamma^2$ is a sufficient to achieve near-optimal performance over the range of parameter values seen in practice (see Table \ref{tab:opt_matching_sim}).

\begin{table*}[ht]
\label{tab:opt_matching_sim}
\centering
\begin{tabular}{|ccc|rrrrrr|r|}
  \hline
 $\alpha$ & $n$ & Predicted & \multicolumn{6}{ c| }{\% average runtime for $r=$} & Misspec. Error \\
 \multicolumn{2}{ |c }{} & Ratio & 1e-4 & 1e-3 & 1e-2 & 0.1 & 1 & 10 &  \\ 
  \hline
 0.001 & 10,000 & 0.047 & 0 & 0 & 36 & 64 & 0 & 0 & 2.2 \\ 
 0.010 & 10,000 & 0.039 & 0 & 0 & 40 & 56 & 4 & 0 & 2.5 \\ 
 0.100 & 10,000 & 0.027 & 0 & 0 & 52 & 40 & 8 & 0 & 4.6 \\ 
 0.001 & 100,000 & 0.015 & 0 & 24 & 76 & 0 & 0 & 0 & 4.3 \\ 
 0.010 & 100,000 & 0.012 & 0 & 48 & 56 & 0 & 0 & 0 & 4.6 \\ 
 0.100 & 100,000 & 0.009 & 0 & 48 & 48 & 4 & 0 & 0 & 7.4 \\ 
   \hline
\end{tabular}
\caption{Simulation for optimal matching of mixing distribution over various choices of Type I error thresholds, $\alpha$, and maximum sample size $n$. We define $r = \gamma^2 / \tau^2$. The Predicted Ratio shows the $\gamma^2$ estimate from (\ref{eq:prior_matching_normal}). The next 6 columns are the proportion of times the fixed $r$ values were empirically found to have lowest average expected run time, $\E_G[T]$. This was done by sampling $200$ experiment sample paths with effect sizes drawn from $G \sim N(0,1)$, and running a mSPRT with various $r$s. The $r$ value with lowest average run time over sample paths was counted to have lowest expected run time for that replication. We perform $B=25$ replications of each parameter combination. The most winning $r$ values coincide well with the estimate in (\ref{eq:prior_matching_normal}). The final column shows the average percent difference between the winning $r$'s estimate of $\E_G[T]$ and the runner-up. A factor of 10 misspecification around the optimal $r$ value results in a less than 10\% increase in average runtime. Comparatively, there is over a factor of 2 difference between the winning and worst $r$ estimates.} 
\end{table*}

\subsection{Improvement over fixed-horizon}

This Bayesian formulation also allows us to compare mSPRT p-values with fixed-horizon testing.  In general, the fixed-horizon sample size must be chosen in reference to the effect sizes where detection is needed; now we can suppose that it is calibrated to have good average power over the prior $G$.

For convenience, we focus on the normal case $G = N(0,\tau^2), H = N(0,\gamma^{2*})$.  We consider two rival tests for an arbitrary goldilocks user: the mSPRT truncated at $M$ and the fixed-horizon test chosen to have the same average power over this prior.  For $\alpha$ small, the former has lower average relative run-length over $G$.
\begin{proposition} \label{prop:improvement}
	Let $\rho(M,\alpha)$ be the average relative run-length of the truncated mSPRT and let $\rho_f(M,\alpha)$ be the relative run-length of the calibrated fixed-horizon test (i.e. the fixed sample size divided by $M$).  If $\alpha \to 0, M \to \infty$, such that $M = O(\log(\alpha^{-1}))$, then $\rho(M,\alpha)/\rho_f(M,\alpha) \to 0$.
\end{proposition}

%{\bf Comparison to fixed horizon testing.} We focus on normal data and a centered normal prior.\footnote{It is possible to extend results to tests on the natural parameter of exponential families, as well as general priors that are positive and continuous on $\Theta$. In fact, some misspecification of $f_\theta$ in (\ref{eq:msprt_definition}) is permitted provided the mean as a function of $\theta$ is correct (see \cite{LS1979})} The results in this section follow from Theorem \ref{thm:ess_truncated}, standard asymptotics of fixed horizon tests, and results of \cite{LS77} and \cite{LS1979}. The following proposition compares the asymptotic Type II error probability, $\beta$, for the mSPRT truncated at $n_S$ versus the UMP fixed horizon test.
%
%\begin{proposition} \label{prop:fast_detection_asymptotic_power}
%Let
%\begin{equation} \nonumber \begin{split}
%C_{S}(\alpha) &= \int_0^1 \Phi \left( \sqrt{ \frac{1}{2} \log \alpha^{-1} } ( x^2 - 1) \right) dx \sim 1 - \frac{1}{\sqrt{ \log \alpha^{-1} } } \\
%C_{f}(\alpha) &= \int_0^1 \Phi \left( \sqrt{ \log \alpha^{-1} } (x - 1 ) \right) dx \in [ 1/2 ,1 ],
%\end{split} 
%\end{equation}
%mSPRT: If $\alpha \rightarrow 0$, $n_S \rightarrow \infty$ such that $\log \alpha^{-1} / n_S \rightarrow 0$,
%\[ \E_{\theta \sim N(\theta_0,\tau)} \{\beta(\theta)\} \sim C_S(\alpha) \frac{2 \sqrt{2}}{\tau} \left( \frac{ \log \alpha^{-1}}{n_S} \right)^{1/2} \]
%Fixed horizon: If $\alpha \rightarrow 0$, $n \rightarrow \infty$ such that $\log \alpha^{-1} / n \rightarrow 0$,
%\[ \E_{\theta \sim N(\theta_0,\tau)} \{\beta(\theta)\} \sim C_f(\alpha) \frac{2 \sqrt{2}}{\tau} \left( \frac{ \log \alpha^{-1}}{n} \right)^{1/2} \]
%\end{proposition}
%\begin{proof}
%Wlog we suppose $\theta_0 = 0$. We begin with the fixed horizon result. It is simple to show that $z_{1 - 2 \alpha} \sim \sqrt{2 \log \alpha^{-1} }$ as $\alpha \rightarrow 0$. Hence
%$$ \beta(\theta) = \bar{\Phi}\left( | \theta| \sqrt{n} - z_{1 - 2\alpha} \right) = \bar{\Phi}\left( ( \log \alpha^{-1} )^{1/2} A_f(\theta,\alpha,n)  \right) $$
%where $A_f(\theta,\alpha,n) = |\theta| \left( \frac{ \log \alpha^{-1}}{n} \right)^{1/2} - \sqrt{2} $.
%
%Let $B_f = \{ \theta \ : \ A_f(\theta,\alpha,n) \geq \sqrt{2} \}$. We split up the expectation as
%$$ \E_{\theta \sim N(0,\tau)} \beta(\theta) = \int_{B_f} \beta(\theta) \frac{1}{\tau} \phi(\theta / \tau) d\theta + \int_{\bar{B}_f} - \beta(\theta) \frac{1}{\tau} \phi(\theta / \tau)d\theta $$
%denoting the two terms by (i) and (ii) respectively. For $\theta \in B_f$, the standard tail bound on the Normal CDF, $\bar{\Phi}(x) \leq x^{-1} \phi(x)$ gives
%\begin{equation} \nonumber
%\begin{split}  \bar{\Phi}\left( ( \log \alpha^{-1} )^{1/2} A_f(\theta,\alpha,n)  \right) &\leq ( 4 \pi \log \alpha^{-1} )^{-1/2} \alpha \\ &= o(\alpha), 
%\end{split}
%\end{equation}
%so that $(i) = o(\alpha)$ as well. For term $(ii)$, we note that $\bar{B}_f \rightarrow \{0\}$ so that $\phi(\theta / \tau) \sim 1$. This, the change of variable $x = \left( \frac{ 2 \log \alpha^{-1}}{n} \right)^{-1/2} \theta$ and symmetry of the integrand give
%\[ (ii) \sim \frac{2 \sqrt{2}}{\tau} \left( \frac{ \log \alpha^{-1}}{n} \right)^{1/2} \int_0^2 \bar{\Phi} \left( ( \log \alpha^{-1} )^{1/2} (x - 1) \right) dx. \] 
%The result follows on noting $ \bar{\Phi} \left( ( \log \alpha^{-1} )^{1/2} (x - 1) \right) = o(1)$ when $x > 1$.
%
%For the mSPRT, we use the normal approximation to $\P_\theta(T(\alpha) > n_S)$ from Theorem 2 of \cite{LS77} which, in the case of standard normal data, gives
%\[ \P_\theta ( T(\alpha) > n_S ) \sim \bar{\Phi} \left\{ ( \log \alpha^{-1} )^{1/2} A_s(\theta,\alpha,n_S) \right\} \]
%where $A_s(\theta,\alpha,n_S) = \frac{1}{2 \sqrt{2}} \left(  \theta^2 \frac{ \log \alpha^{-1}}{n_S}  - 2 \right)$. The rest of the proof proceeds as for the fixed horizon test, except with $B_s = \{ \theta \ : \ A_s(\theta,\alpha,n) \geq \sqrt{2} \}$ and changes in the integrand of $(ii)$ as stated in the proposition.
%\end{proof}
%
%Thus similar asymptotic power can be achieved by $n_{S} = \left( C_{S}(\alpha) / C_{f}(\alpha) \right)^{2} n = O(n)$. However, while the fixed horizon test must wait for all $n$ samples, the truncated mSPRT typically stops much earlier.
%
%\begin{theorem} \label{prop:fast_detection_asymptotic_sample_size}
%Let $\alpha \rightarrow 0$, $n_S \rightarrow \infty$ such that $\log \alpha^{-1} / n_S \rightarrow 0$ and ,
%\[  \E_{\theta \sim N(0,\tau)} \{ \E_\theta ( T_{n_S}^\alpha ) \} = o(n_S) \]
%up to terms which are $o(1)$.
%\end{theorem}
%\begin{proof}
%Again we take $\theta_0 = 0$ wlog, so for standard normal data $I(\theta, 0) = \theta^2 / 2$. Invoking Theorem \ref{thm:ess_truncated}, we attack the two terms separately. Let $\delta = ( 2 n_S^{-1} \log \alpha^{-1} )^{1/2}$.
%\[ Pr_{\theta \sim N(0,\tau)} ( \bar{A}_{n_S} ) = 2 \int_0^\delta \frac{1}{\tau} \phi(\theta / \tau ) d \theta \sim \frac{2 \sqrt{2}}{\tau} \left( \frac{ \log \alpha^{-1}}{n_S} \right)^{1/2}\]
%by similar arguments to those in the proof of Proposition \ref{prop:fast_detection_asymptotic_power}.
%
%The first term in Theorem \ref{thm:ess_truncated} is more complicated. By equation (67) of \cite{LS1979} and the discussion following,
%\begin{equation} \label{exp_time_decomp}
%\begin{split}  \E_\theta ( T(\alpha) ) &= 2 \theta^{-2} \log \alpha^{-1} + \theta^{-2} \log \log \alpha^{-1} + D_1 \theta^{-2} \log | \theta | \\
%&+ D_2 \theta^{-2} + D_3 + D_4 \theta^{-1} B( \theta / 2) + o(1) 
%\end{split}
%\end{equation}
%as $\alpha \rightarrow 0$, where 
%\[ B(u) = \sum_{k = 1}^{\infty} k^{-1/2} \phi( u k^{1/2} ) - u \Phi ( - u k^{1/2} ). \]
%It remains to show that each term in \ref{exp_time_decomp} has $o(n_S)$ expectation on $1_{A_{n_S}}$. We focus on terms 1, 3 \& 6 as the remainder are clearly lower order.
%\begin{enumerate}
%\item[Term 1.]
%We note that, for any $n_S$,
%$$ \E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-2} ) = 4 \int_\delta^\infty \theta^{-2} \frac{1}{\tau} \phi( \frac{\theta}{ \tau}) d \theta = \frac{4}{\tau^2} \left( \frac{\tau}{\delta} \phi( \frac{\delta}{\tau} ) - \bar{\Phi}( \frac{\delta}{\tau} ) \right) $$
%which is bounded over $\alpha \in (0, 1 - \epsilon)$. It follows that
%\[  \E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-2} ) \log \alpha^{-1} \sim \frac{ 2 \sqrt{2} }{\tau} n_S \left( \frac{ \log \alpha^{-1}}{n_S} \right)^{1/2} = o(n_S). \]
%\item[Term 3.] By calculus, 
%\begin{equation} \nonumber \begin{split}
% &\E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-2} \log | \theta | \} \propto \int_\delta^\infty \theta^{-2} \log \theta e^{-\theta^2 / 2 \tau^2 } \\
% &= \frac{1}{4} \left[ \frac{1}{\sqrt{2} \tau} \Gamma \left( - \frac{1}{2} \ , \ \frac{\delta^2}{2 \tau^2} \right) \log \delta \right. \\
% &+ \left. \delta^{-1} \text{MeijerG} \left( \{ \{\}, \{ \frac{3}{2} , \frac{3}{2} \} , \{ \{0,\frac{1}{2},\frac{1}{2}\},\{\}\} , \frac{\delta^2}{2 \tau^2} \right) \right],
% \end{split} \end{equation}
%The $\text{MeijerG}$ term is asymptotically constant as $\delta \rightarrow 0$, and
%\[ \Gamma \left( - \frac{1}{2} \ , \ \frac{\delta^2}{2 \tau^2} \right) \rightarrow 2 \sqrt{2} \tau \delta^{-1}. \]
%It follows that
%$$ \E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-2} \log | \theta | ) \propto n_S \left[ K_1 \left( n_S \log \alpha^{-1} \right)^{-1/2} + K_2 \left( \frac{ \delta \log \delta }{\log \alpha^{-1}} \right) \right] $$
%where $K_i$ are both constants depending on $\tau$. Both terms in the bracketed sum clearly converge to $0$ since $\delta \rightarrow 0$.
%\item[Term 6.] By standard bounds on the normal CDF, $B(u) \geq 0$ and 
%\begin{equation} \nonumber \begin{split} &B(u) \leq u^{-2} \left( \int_1^\infty x^{-3/2} \phi(u x^{1/2}) dx + \phi(u) \right) \\
%&= \theta^{-2} \left( 3 \phi(\theta) - 2 \theta \Phi( - \theta ) \right) 
%  \end{split} \end{equation}
%Hence,
%\begin{equation} \nonumber \begin{split}  \E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-1} B( \theta / 2)) \leq K_3 \, \E_{\theta \sim N(0,\tau)} ( \v{1}_{A_{n_S}} \theta^{-3} \phi(\theta / 2) ) + K_4 \\
%\leq K_4 \delta^{-2} e^{K_5 \delta^2} - K_7 \Gamma(0, K_6 \delta^2 ) + K_4,
%\end{split}\end{equation}
%where $\delta^{-2} = n_S / \log \alpha^{-2} = o(n_S)$ and $\Gamma(0, K_6 \delta^2 ) \sim \log K_6 / \delta^2 = O( \log \delta ) = o(n_S)$.
%\end{enumerate}
%\end{proof}
%
%Finally we note that, in addition to the improvement in average efficiency provided by mSPRTs over fixed horizon testing, our new methodology allows the user to change $\alpha$ and $n_S$ mid-experiment to accomodate dynamic exogenous demands.

